Do Informational Cascades Happen with Non-myopic Agents?

We consider an environment where players need to decide whether to buy a certain product (or adopt a technology) or not. The product is either good or bad, but its true value is unknown to the players. Instead, each player has her own private information on its quality. Each player can observe the previous actions of other players and estimate the quality of the product. A classic result in the literature shows that in similar settings informational cascades occur where learning stops for the whole network and players repeat the actions of their predecessors. In contrast to this literature, in this work, players get more than one opportunity to act. In each turn, a player is chosen uniformly at random from all players and can decide to buy the product and leave the market or wait. Her utility is the total expected discounted reward, and thus myopic strategies may not constitute equilibria. We provide a characterization of perfect Bayesian equilibria (PBE) with forward-looking strategies through a fixed-point equation of dimensionality that grows only quadratically with the number of players. Using this tractable fixed-point equation, we show the existence of a PBE and characterize PBE with threshold strategies. Based on this characterization we study informational cascades in two regimes. First, we show that for a discount factor {\delta} strictly smaller than one, informational cascades happen with high probability as the number of players N increases. Furthermore, only a small portion of the total information in the system is revealed before a cascade occurs ...

==> Non-myopic Information Cascades _ Review Response/achilleas_bio.tex <==



%\begin{IEEEbiography}{Achilleas Anastasopoulos}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/AA.jpg}}]{Achilleas Anastasopoulos}
%
(S'97-M'99-SM'13) was born in Athens, Greece in 1971. He received the Diploma
in Electrical Engineering from the National Technical University of
Athens, Greece in 1993, and the M.S.\ and Ph.D.\ degrees in Electrical
Engineering from University of Southern California in 1994 and 1999,
respectively. He is currently an Associate Professor at the University of
Michigan, Ann Arbor, Department of Electrical Engineering and Computer
Science.

His research interests lie in the general area of communication and information theory,
with emphasis in channel coding and multi-user channels;
control theory with emphasis in decentralized stochastic control and its
connections to communications and information theoretic problems;
analysis of dynamic games and mechanism design for resource allocation on networked systems.

He is the co-author
of the book \emph{Iterative Detection: Adaptivity, Complexity Reduction,
and Applications,} (Reading, MA: Kluwer Academic, 2001).

Dr.\ Anastasopoulos is the recipient of the ``Myronis Fellowship'' in
1996 from the Graduate School at the University of Southern California,
the NSF CAREER Award in 2004,
and was a co-author for the paper that received the best student paper award in ISIT 2009.
%
He served as a technical program committee member for 
ICC 2003, 2015--2018; 
Globecom 2004, 2012; 
VTC 2007, 2014, 2015; 
ISIT 2015,
SPAWC 2018,
and is currently serving as the TPC co-Chair for the Communication Theory Symposium, ICC'21.
He was an associate editor for the IEEE Transactions on Communications in 2003--2008.
%and
%is currently serving as an associate editor for Communications in the IEEE Transactions on Information Theory.
%

%
\end{IEEEbiography}
\vfill





==> Non-myopic Information Cascades _ Review Response/ilai_bio.tex <==



%\begin{IEEEbiography}{Achilleas Anastasopoulos}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/ilai.png}}]{Ilai Bistritz}
%
received his B.Sc. in 2012 (magna cum laude) and his M.Sc in 2016 (summa cum laude), both in Electrical Engineering and both from Tel-Aviv University, Israel. He is currently working toward a Ph.D. in Electrical Engineering at Stanford University, Stanford, CA, USA. His main research interests are game theory, decision-making over networks and multiagent learning.

\end{IEEEbiography}
\vfill





==> Non-myopic Information Cascades _ Review Response/nas_bio_ieee.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Nasimeh.png}}]{Nasimeh Heydaribeni}
	%
	received her B.S. and M.S. degrees in Electrical Engineering at Sharif University of Technology, Tehran, Iran, in 2015 and 2017, respectively. She is currently pursuing her Ph.D. degree in Electrical Engineering and Computer Science at University of Michigan, Ann Arbor. Her research interests are game theory and its applications in networked systems with emphasis on mechanism design, dynamic games with asymmetric information and information design.
\end{IEEEbiography}
\vfill

